SimPLR: A Simple and Plain Transformer for Efficient Object Detection and Segmentation

The ability to detect objects in images at varying scales has played a pivotal role in the design of modern object detectors. Despite considerable progress in removing hand-crafted components and simplifying the architecture with transformers, multi-scale feature maps and pyramid designs remain a key factor for their empirical success. In this paper, we show that shifting the multiscale inductive bias into the attention mechanism can work well, resulting in a plain detector `SimPLR' whose backbone and detection head are both non-hierarchical and operate on single-scale features. We find through our experiments that SimPLR with scale-aware attention is plain and simple architecture, yet competitive with multi-scale vision transformer alternatives. Compared to the multi-scale and single-scale state-of-the-art, our model scales better with bigger capacity (self-supervised) models and more pre-training data, allowing us to report a consistently better accuracy and faster runtime for object detection, instance segmentation, as well as panoptic segmentation. Code is released at https://github.com/kienduynguyen/SimPLR.

==> sec/background.tex <==
\section{Background}
\label{sec:background}
Our goal is to further simplify the detection and segmentation pipeline from~\cite{zhu2021deformable,li2022vitdet,nguyen2022boxer}, and to prove the effectiveness of the plain detector in \textit{both} object detection and segmentation tasks. To do so, we focus on the recent progress in end-to-end detection and segmentation. As a result, we utilize the sparse attention mechanism, Box-Attention in~\cite{nguyen2022boxer}, as strong baselines due to its effectiveness in learning discriminative object representations while being lightweight in computation.

% Given the input feature map from the backbone, the encoder layers with the sparse attention mechanism will output contextual representations. The contextual representations are utilized to predict object proposals and to initialize object queries for the decoder. We denote the input feature map of an encoder layer as $e \in \mathbb{R}^{H_e \times W_e \times d}$ and the query vector $q \in \mathbb{R}^d$, with $H_e, W_e, d$ denoting height, width, and dimension of the input features respectively. 

In box-attention, each query vector $q \in \mathbb{R}^d$ in the input feature map is assigned an anchor $r {=} [x, y, w, h]$, where $x, y$ indicate the query coordinate and $w, h$ are the size of the anchor. The box-attention refines the anchor into a region of interest.
%
% \begin{equation}
%     r' = F_\text{scale}\big(F_\text{translate}(r, q), q\big), 
% \end{equation}
% \begin{equation}
%     F_\text{scale}(r, q) = [x, y, w + \Delta_w, h + \Delta_h], 
% \end{equation}
% \begin{equation}
%     F_\text{translate}(r, q) = [x + \Delta_x, y + \Delta_y, w, h],
% \end{equation}
% %
% where $F_\text{scale}$ and $F_\text{translate}$ are the scaling and translation transformations, $\Delta_x, \Delta_y, \Delta_w$ and $\Delta_h$ are the offsets regarding to the reference window $r$. A linear projection ($\mathbb{R}^d \rightarrow \mathbb{R}^{4}$) is applied on $q$ to predict offset parameters (\ie, $\Delta_x, \Delta_y, \Delta_w$ and $\Delta_h$) \wrt the window size.
%
During the attention head computation, a $2 {\times} 2$ feature grid is sampled from the corresponding region of interest, resulting in a set of value features $v_i \in \mathbb{R}^{2 \times 2 \times d_h}$. The $2 {\times} 2$ attention scores are efficiently generated by computing a dot-product between $q \in \mathbb{R}^d$ and relative position embeddings ($k_i \in \mathbb{R}^{2 \times 2 \times d}$) followed by a $\softmax$ function. The attended feature $\mathrm{head}_i \in \mathbb{R}^{d_h}$ is a weighted sum of $2 {\times} 2$ value features in $v_i$ with the corresponding attention weights:
%
% \begin{equation}
%     \alpha =  \softmax(q^{\top} {k_i}),
% \end{equation}
% \begin{equation}
%     \mathrm{head}_i = \mathop{\mathrm{\boxattnop}}(q, k_i, v_i) = \sum_{j=0}^{2 \times 2} \alpha_j v_{i_j},
% \end{equation}
%
where $q \in \mathbb{R}^d$, $k_i \in \mathbb{R}^{2 \times 2 \times d}$, $v_i \in \mathbb{R}^{2 \times 2 \times d_h}$ are query, key and value vectors of box-attention, $\alpha_j$ is the $j$-th attention weight, and $v_{i_j}$ is the $j$-th feature vector in the feature grid $v_i$. To better capture objects at different scales, the box-attention~\cite{nguyen2022boxer} takes $t$ multi-scale feature maps, $\{e^j\}_{j=1}^t$, as its inputs in order to produce $\mathrm{head}_i$.

% \paragraph{Multi-head Deformable Attention.} In deformable attention, each query vector $q \in \mathbb{R}^d$ is assigned a reference point $p=[x,y]$, where $x,y$ indicate the query coordinate normalized by the image size. The deformable attention attends to points of interest around the query coordinate, $p'$, as:
% %
% \begin{equation}
%     p' = F_\text{deform}(p, q) = [x + \Delta_x, y + \Delta_y],
% \end{equation}
% %
% where $F_\text{deform}$ is the deformable function, $\Delta_x,\Delta_y$ are the offets regarding to the reference point $p$. Similarly, a linear projection ($\mathbb{R}^d \rightarrow \mathbb{R}^2$) is applied on $q$ to predict offset paramters \wrt the reference point.

% During the $i$-th attention head computation, the deformable attention predicts a set of 4 points, resulting in value features $v_i \in \mathbb{R}^{4\times d_h}$. The $4$ attention scores are generated by applying another linear projection, $g_i: \mathbb{R} \rightarrow \mathbb{R}^4$, on $q$ followed by a $\softmax$ function. The attended feature $\mathrm{head}_i \in \mathbb{R}^{d_h}$ is a weighted sum of $4$ value features in $v_i$ with the corresponding attention weights:
% %
% \begin{equation}
%     \alpha =  \softmax\big(g_i(q)\big),
% \end{equation}
% \begin{equation}
%     \mathrm{head}_i = \mathop{\mathrm{\deformattnop}}(q, v_i) = \sum_{j=0}^{4} \alpha_j v_{i_j},
% \end{equation}
% %
% where $q \in \mathbb{R}^d$, $v_i \in \mathbb{R}^{2 \times 2 \times d_h}$ are query, value vectors of deformable attention, $\alpha_j$ is the $j$-th attention weight, and $v_{i_j}$ is the $j$-th feature vector in the value $v_i$. The deformable attention~\cite{zhu2021deformable} also utilizes $t$ multi-scale feature maps, $\{e^j\}_{j=1}^t$, as its inputs in order to produce $\mathrm{head}_i$.


The sparse attention like box-attention and deformable attention lies at the core of recent end-to-end detection and segmentation models due to its ability of capturing object information with lower complexity. The effectiveness and efficiency of these attention mechanisms bring up the question: \textit{Is multi-scale object information learnable within the detector which is non-hierarchical and single-scale?}


==> sec/background_legacy.tex <==
\section{Background}
\label{sec:background}
Our goal is to further simplify the detection and segmentation pipeline from~\cite{zhu2021deformable,li2022vitdet,nguyen2022boxer}, and to prove the effectiveness of the plain detector in object detection and segmentation tasks. To do so, we focus on the recent progress in end-to-end detection and segmentation. Specifically, we utilize the box-attention mechanism by~\cite{nguyen2022boxer} as a strong baseline due to its effectiveness in learning discriminative object representations while being lightweight in computation. 

Given the input feature map from the backbone, the encoder layers with box-attention will output contextual representations. The contextual representations are utilized to predict object proposals and to initialize object queries for the decoder. We denote the input feature map of an encoder layer as $e \in \mathbb{R}^{H_e \times W_e \times d}$ and the query vector $q \in \mathbb{R}^d$, with $H_e, W_e, d$ denoting height, width, and dimension of the input features respectively. Each query vector $q \in \mathbb{R}^d$ in the input feature map is assigned a reference window $r {=} [x, y, w, h]$, where $x, y$ indicate the query coordinate and $w, h$ are the size of the reference window both being normalized by the image size. The box-attention refines the reference window into a region of interest, $r'$, as:
%
\begin{equation}
    r' = F_\text{scale}\big(F_\text{translate}(r, q), q\big), 
\end{equation}
\begin{equation}
    F_\text{scale}(r, q) = [x, y, w + \Delta_w, h + \Delta_h], 
\end{equation}
\begin{equation}
    F_\text{translate}(r, q) = [x + \Delta_x, y + \Delta_y, w, h],
\end{equation}
%
where $F_\text{scale}$ and $F_\text{translate}$ are the scaling and translation transformations, $\Delta_x, \Delta_y, \Delta_w$ and $\Delta_h$ are the offsets regarding to the reference window $r$. A linear projection ($\mathbb{R}^d \rightarrow \mathbb{R}^{4}$) is applied on $q$ to predict offset parameters (\ie, $\Delta_x, \Delta_y, \Delta_w$ and $\Delta_h$) \wrt the window size.

Similar to self-attention~\cite{vaswani2017transformer}, box-attention aggregates $n$ multi-head features from regions of interest:
%
\begin{equation}
\label{eq:multihead}
    \mathop{\mathrm{MultiHeadAttention}} = \mathop{\mathrm{Concat}}(\mathrm{head}_1, \ldots, \mathrm{head}_n) \, W^O,
\end{equation}
%
During the $i$-th attention head computation, a $2 {\times} 2$ feature grid is sampled from the corresponding region of interest $r'_i$, resulting in a set of value features $v_i \in \mathbb{R}^{2 \times 2 \times d_h}$. The $2 {\times} 2$ attention scores are efficiently generated by computing a dot-product between $q \in \mathbb{R}^d$ and relative position embeddings ($k_i \in \mathbb{R}^{2 \times 2 \times d}$) followed by a $\softmax$ function. The attended feature $\mathrm{head}_i \in \mathbb{R}^{d_h}$ is a weighted average of the $2 {\times} 2$ value features in $v_i$ with the corresponding attention weights:
%
\begin{equation}
    \alpha =  \softmax(q^{\top} {k_i}),
\end{equation}
\begin{equation}
    \mathrm{head}_i = \mathop{\mathrm{\boxattnop}}(q, k_i, v_i) = \sum_{j=0}^{2 \times 2} \alpha_j v_{i_j},
\end{equation}
%
where $q \in \mathbb{R}^d$, $k_i \in \mathbb{R}^{2 \times 2 \times d}$, $v_i \in \mathbb{R}^{2 \times 2 \times d_h}$ are query, key and value vectors of box-attention, $\alpha_j$ is the $j$-th attention weight, and $v_{i_j}$ is the $j$-th feature vector in the feature grid $v_i$. To better capture objects at different scales, the box-attention~\cite{nguyen2022boxer} takes $t$ multi-scale feature maps, $\{e^j\}_{j=1}^t$, as its inputs. In the $i$-th attention, $t$ feature grids are sampled from each of multi-scale feature maps in order to produce $\mathrm{head}_i$.

By computing the attended feature within regions of interest in each attention head, box-attention shows strong performance in object detection and instance segmentation with a small computational budget. The transformation functions (\ie, translation and scaling) allow box-attention to capture long-range dependencies. The effectiveness and efficiency of box-attention mechanism brings up the question: \textit{Is multi-scale object information learnable within a single-scale feature map?}


==> sec/method_legacy.tex <==
\section{\ours: A Simple and Plain Detector}
\label{sec:simplr}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/compare1.pdf}\\
    \caption{
    \textbf{Object detection architectures. Left:} The plain-backbone detector from~\cite{li2022vitdet} whose input (denoted in the dashed region) are multi-scale features. \textbf{Middle:} State-of-the-art end-to-end detectors~\cite{nguyen2022boxer,cheng2022mask2former} utilize a hierarchical backbone (\ie, Swin~\cite{liu2021swintransformer}) to create multi-scale inputs. \textbf{Right:} Our simple single-scale detector following the end-to-end framework. Where existing detectors require feature pyramids to be effective, we propose a plain detector, \ours, whose backbone and detection head are non-hierarchical and operate on a single-scale feature map. The plain detector, \ours, achieves on par or even better performance compared to hierarchical and/or multi-scale counterparts while being more efficient.
    % We show through our experiments that \ours also shows good scaling behaviour and effectively takes advantages from a significant progress of self-supervised learning with ViTs.
    }\label{fig:compare}
\end{figure*}

Multi-scale feature maps in a hierarchical backbone can be easily extracted from the pyramid structure~\cite{wei2016ssd,tsung2017fpn,zhu2021deformable}. When moving to a ViT backbone with a constant feature resolution, the creation of multi-scale feature maps requires complex backbone adaptations. Moreover, the benefits of multi-scale features in object detection frameworks using ViTs remain unclear. Recent studies on plain-backbone detection~\cite{li2022vitdet,chen2022uvit} conjecture the high-dimensional ViT with self-attention and positional embeddings~\cite{vaswani2017transformer} is able to preserve important information for localizing objects\footnote{ViT-B and larger ($\text{dim}\ge768$) can maintain information with a patch size of $16{\times}16{\times}3$ in the input image.}. From this conjecture, we hypothesize that a proper design of the transformer-based head will enable a plain detector.

Our proposed detector, \ours, is conceptually simple: a pre-trained ViT backbone to extract plain features from an image, which are then fed into a single-scale encoder-decoder to make the final prediction (See \cref{fig:compare}). Thus, \ours is a natural idea as it eliminates the non-trivial creation of feature pyramids from the ViT backbone. But the single-scale encoder-decoder requires an effective design to deal with objects at different scales. Next, we introduce the key elements of \ours, including its \emph{scale-aware} attention that is the main factor for learning of adaptive object scales.


\boldparagraph{Network Architecture.} \ours follows the end-to-end detection and segmentation framework proposed by~\cite{zhu2021deformable,nguyen2022boxer} with the two-stage design. Specifically, we use a plain ViT as the backbone with $14\times14$ windowed attention and four equally-distributed global attention blocks as in~\cite{li2022vitdet}. In the detection head, the \ours encoder receives input features via a projection of the last feature map from the ViT backbone. The object proposals are then predicted using single-scale features from the encoder and top-scored features are initialized as object queries for the \ours decoder to predict bounding boxes and masks. Note this design differs from most state-of-the-art systems~\cite{cheng2022mask2former,li2022vitdet,lin2023plaindetr}, where the feature pyramids are essential for object proposal generation and/or final prediction. Our approach follows the spirit of ViT~\cite{dosovitskiy2021vit} that applies a single and constant feature resolution throughout the detection head, which turns out to largely simplify the architectural choices and remove handcrafted components compared to Swin~\cite{liu2021swintransformer} or MViT~\cite{fan2021mvit}.

Formally, we apply a projection $f$ to the last feature map of the pre-trained ViT backbone, resulting in the input feature map $e \in \mathbb{R}^{H_e \times W_e \times d}$ where $H_e, W_e$ are the size of the feature map, and $d$ is the hidden dimension of the detection head. In \ours, the projection $f$ is simply a single convolution projection, that provides us a great flexibility to control the resolution and dimension of the input features $e$ to the encoder. The projection allows \ours to decouple the feature scale and dimension between its backbone and detection head. To be specific, the ViT backbone with global self-attention can operate efficiently on high-dimensional and low-resolution features, while the transformer-based detection head with sparse attention takes the lower dimension but higher resolution input for better object prediction. This practice is different from the creation of SimpleFPN in~\cite{li2022vitdet} where a different stack of multiple convolution layers is used for each feature scale (more details shown in Fig. A in the supplementary material). We show by experiments that this formulation is key for plain detection and segmentation while keeping our network efficient.

\boldparagraph{Scale-aware attention.} The output features of the encoder should capture objects at different scales. Therefore, unlike the feature pyramids where each set of features encode a specific scale, predicting objects from a plain feature map requires its feature vectors to reason about dynamic scale information based on the image content. This can be addressed effectively by a multi-head attention mechanism that capture different scale information in each of its attention heads. 
In that case, global self-attention is a potential candidate because of its large receptive field and powerful representation. However, its computational complexity is quadratic \wrt the sequence length of the input, making the operation computationally expensive when dealing with high-resolution images. The self-attention also leads to worse performance and slow convergence in end-to-end detection~\cite{zhu2021deformable}. This motivated us to develop a multi-head \emph{scale-aware} attention mechanisms based on sparse attention such as box-attention and deformable attention.

The multi-head attention mechanism, proposed by~\cite{vaswani2017transformer}, is a core operation in the transformer architectures for capturing diverse patterns given a query vector in the input features. In the multi-head box-attention~\cite{nguyen2022boxer}, each feature vector is assigned a reference window which is then refined to locate a region-of-interest in each attention head via scaling and translation transformations. Theoretically, the scaling transformation should provide box-attention the capability to learn multi-scale regions-of-interest in multiple attention heads. However, we find in our experiments that the scaling function in box-attention only performs minor modifications regarding to its reference window. As a result, feature vectors learn to adapt to a specific scale of the reference window assigned to them. While this behaviour may not impact the multi-scale box-attention -- which utilizes feature pyramids for detecting objects -- it poses a big challenge in learning scale-equivariant features on a single-scale input.

To address this limitation, we propose two variants of multi-head \emph{scale-aware} attention (\ie, \emph{fixed-scale} and \emph{adaptive-scale}) that integrate different scales into each attention head, allowing query vectors to choose the suitable scale information during training. Our proposed attention mechanism is simple: we assign reference windows of $m$ different scales to attention heads of each query. We use $m$ reference windows with size $w {=} h \in \{s \cdot 2^j\}_{j=0}^{m-1}$, where $s$ is the size of the smallest window, and $m$ is the number of scales with the growing rate of $2$. Surprisingly, our experiments show that the results are not sensitive to the size of the window, as long as \emph{enough} number of scales are used.
%
\begin{enumerate}[leftmargin=*,itemsep=0pt,topsep=0pt]
    \item[i)] \emph{Fixed-Scale Attention.} Given reference windows of $m$ scales, we distribute them to $n$ attention heads in a round-robin manner. Thus, in multi-head fixed-scale attention, $\frac{n}{m}$ attention heads are allocated for each of the window scales. This uniform distribution of different scales enables fixed-scale attention to learn diverse information from local to more global context. The aggregation of $n$ heads results in scale-aware features, that is suitable for predicting objects of different sizes.
    \item[ii)] \emph{Adaptive-Scale Attention.} Instead of uniformly assigning $m$ scales to $n$ attention heads, the adaptive-scale attention learns to allocate a scale distribution based on the context of the query vector. This comes from the motivation that the query vector belonging to a small object should use more attention heads for capturing fine-grained details rather than global context, and vice versa. More specifically, in each attention head, the adaptive-scale attention predicts offsets for all reference windows of $m$ scales and samples feature grids from $m$ regions-of-interest. Given the query vector $q \in \mathbb{R}^d$, it then applies a learnable projection on $q$ followed by $\softmax$ normalization to generate attention scores which allow it to focus on the feature grid of suitable scale. The adaptive-scale attention provides efficiency due to sparse sampling and strong flexibility to control scale distribution via its attention computation.
\end{enumerate}

\boldparagraph{Plain backbone.} \ours deploys ViT as its plain backbone for feature extraction. We show that \ours can take advantages of recent progress in self-supervised learning with ViTs. To be specific, \ours generalizes to ViT backbones initialized by MAE~\cite{he2022mae} and BEiTv2~\cite{peng2022beitv2}. The efficient design of \ours allows us to effectively scale to larger ViT backbones which recently show to be even more powerful in learning representations~\cite{he2022mae,zhai2022scalingvit,dehghani2023scalingvit22b}. We also provide the comparison between different pre-training approaches of the \ours backbone in the supplementary material.

\boldparagraph{Adaption for panoptic segmentation.} Panoptic segmentation proposed by~\cite{kirillov2019panoptic} requires the network to segment both ``thing'' and ``stuff''.
To enable the plain detector on panoptic segmentation, we make an adaptation in the mask prediction of \ours. To be specific, we predict segmentation masks of both types by computing the dot-product between object queries and a feature map following~\cite{cheng2022mask2former}. We provide a brief description on these modifications, the full implementation details are provided in the supplementary material.

In~\cite{cheng2022mask2former}, the $\frac{1}{4}$ feature scale is extracted from the first stage of the Swin and combined with upscaled $\frac{1}{8}$ features from the last layer of the encoder for the mask prediction. As the ViT and SimPLR encoder features are of lower resolution, we simply interpolate the last encoder layer to $\frac{1}{4}$ scale and add a single attention layer on top. This simple modification produces a high resolution feature map that is beneficial for learning fine-grained details.
%
Masked instance-attention follows the dense grid sampling strategy (\eg, $14\times14$ feature grid) of box-attention in the decoder~\cite{nguyen2022boxer}, but differs in the computation of the attention scores to better capture objects of different shapes. Inspired by masked self-attention~\cite{cheng2022mask2former}, we employ the masking to $14\times14$ attention scores of the feature grid based on the mask prediction scores in the previous decoder layer. By focusing better on foreground features, the decoder yields more discriminative features.

% Our goal is to have \emph{minimal} adaptation which allows us to use the same training recipe for all tasks, including object detection, instance segmentation, and panoptic segmentation. As the output feature of our encoder is in $\frac{1}{8}$ scale of the original image, we simply use a transposed convolution layer to generate the high-resolution feature for mask prediction. We found that it is beneficial to stack $K$ encoder layers on top of the high-resolution feature to learn more contextual information. In addition, we incorporate the decoder with masked instance-attention to obtain discriminative representation for mask prediction. Different from masked cross-attention in~\cite{cheng2022mask2former}, our masked instance-attention extends box-attention in~\cite{nguyen2022boxer} which yields a small complexity when dealing with feature map of $\frac{1}{8}$ scale from the encoder. More details are provided in the supplementary document.

% \boldparagraph{Masked instance-attention.} The masked instance-attention follows the grid sampling strategy of the box-attention in~\cite{nguyen2022boxer}, but differs in the computation of attention scores to better capture objects of different shapes. To be specific, the region of interest $r'_i$ is divided into 4 bins of $2 \times 2$ grid, each of which contains a $\frac{m}{2} \times \frac{m}{2}$ grid features sampled using bilinear interpolation. Instead of assigning an attention weight to each feature vector, a linear projection ($\mathbb{R}^d \rightarrow \mathbb{R}^{2 \times 2}$) is adopted to generate the $2 \times 2$ attention scores for 4 bins. The $\frac{m}{2} \times \frac{m}{2}$ feature vectors within the same bin share the same attention weight. This is equivalent to the \textit{average} aggregation of feature values covered by each bin, which shows to reduce misalignments in RoIAlign~\cite{he2017maskrcnn}:
% \begin{equation}
%     \mathrm{head}_i = \sum_{k=0}^{2 \times 2} \sum_{j=0}^{\frac{m}{2} \times \frac{m}{2}} \frac{\alpha_k}{\frac{m}{2} \cdot \frac{m}{2}} \, v_{i_{k,j}},
% \end{equation}
% where $a_k$ is the attention weight corresponding to $k$-th bin and $v_{i_{k,j}}$ is the $j$-th feature vector inside $k$-th bin.


% Inspired by~\cite{cheng2022mask2former}, we utilize the mask prediction before the $\sigmoid$ of the previous decoder layer $\mathcal{M}_q \in \mathbb{R}^{H_m \times W_m}$ corresponding to the object query $q$. Given the coordinates of grid features within the region of interest $r'_i$, we sample the corresponding mask scores using bilinear interpolation. The sampled mask scores are binarized with the 0.5 threshold and applied into the attention computation.
% %
% \begin{align}
%     \mathrm{head}_i &= \sum_{k=0}^{2 \times 2} \sum_{j=0}^{\frac{m}{2} \times \frac{m}{2}} \Big(\frac{\alpha_k}{\frac{m}{2} \cdot \frac{m}{2}} + m_{i_{k,j}} \Big) \, v_{i_{k,j}} , \\
%     m_{i_{k,j}} &= 
%         \begin{cases}
%         0 & \text{if } \sigmoid\Big(\mathcal{M}_q\big(v_{i_{k,j}}\big)\Big) \geq 0.5 \\
%         -\infty & \text{otherwise} \\
%         \end{cases}   ,
% \end{align}
% %
% where $\mathcal{M}_q\big(v_{i_{k,j}}\big)$ is the mask score sampled at the location of the feature $v_{i_{k,j}}$. The masked instance-attention along with high-resolution layers allow \ours to capture more fine-grained details, which is beneficial for panoptic segmentation.


==> sup/abstract.tex <==
This supplementary material provides: 1) implementation details; 2) additional results; 3) qualitative results; and 4) license information.

==> sup/additional.tex <==

  
\section{Additional Results}

\begin{table}[h]
    \centering
    \footnotesize
    % \floatbox[{\capbeside\thisfloatsetup{capbesideposition={top,right}}}]{table}[\FBwidth]
    {
    \tablestyle{4.5pt}{1.2}
    \begin{tabular}{lcccccc}
    \multicolumn{1}{l|}{method} & backbone & \multicolumn{1}{c|}{pre-train} & PQ & PQ$^\text{th}$ & \multicolumn{1}{c|}{PQ$^\text{st}$} & FPS \\
    \shline
    \rowcolor{orange!50} \textbf{Feature pyramids} &  &  &  &  &  &  \\
    \multicolumn{1}{l|}{MaskFormer~\citep{cheng2021maskformer}} & Swin-B & \multicolumn{1}{c|}{sup-1K} & 51.1 & 56.3 & \multicolumn{1}{c|}{43.2} & - \\
    \multicolumn{1}{l|}{Mask2Former~\citep{cheng2022mask2former}} & Swin-B & \multicolumn{1}{c|}{sup-1K} & 55.1 & 61.0 & \multicolumn{1}{c|}{46.1} & 7 \\
    \hline
    \rowcolor{orange!50} \textbf{Plain detector} &  &  &  &  &  &  \\
    \multicolumn{1}{l|}{\ours} & ViT-B & \multicolumn{1}{c|}{sup-1K} & \textbf{55.5} & \textbf{61.4} & \multicolumn{1}{c|}{\textbf{46.2}} & \textbf{13} \\
    \end{tabular}
    }
    {
        \caption{\textbf{More panoptic segmentation comparison} between \ours with ViT-B backbone and other methods with Swin-B backbone. All backbones are pre-trained on ImageNet-1K with supervised pre-training. \ours still shows competitive results when using only single-scale input.}\label{tab:more_panop}
    }%
\end{table}
  
\boldparagraph{More panoptic segmentation comparison.} Here, we provide more results of \ours with ViT-B backbone and other methods with Swin-B backbone using supervised pre-training on COCO panoptic segmentation in \cref{tab:more_panop}. \ours continues to show strong segmentation performance when using only single-scale input.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[h]
%     \centering
%     \footnotesize
%     % \floatbox[{\capbeside\thisfloatsetup{capbesideposition={top,right}}}]{table}[\FBwidth]
%     {
%     \tablestyle{8pt}{1.2}
%     \begin{tabular}{lcccc}
%     \multicolumn{1}{l|}{method} & backbone & \multicolumn{1}{c|}{pre-train} & PQ \\
%     \shline
%     \rowcolor{orange!50} \textbf{Feature pyramids} &  &  & \\
%     \multicolumn{1}{l|}{Panoptic FCN~\citep{li2021panopticfcn}} & Swin-L & \multicolumn{1}{c|}{sup-21K} & 65.9  \\
%     \multicolumn{1}{l|}{Panoptic DeepLab~\citep{cheng2020panoptic}} & SWideRNet~\citep{chieh2020wideresnet} & \multicolumn{1}{c|}{sup-1K} & 66.4  \\
%     \multicolumn{1}{l|}{Mask2Former~\citep{cheng2022mask2former}} & Swin-B & \multicolumn{1}{c|}{sup-21K} & 66.1 \\
%     \multicolumn{1}{l|}{Mask2Former~\citep{cheng2022mask2former}} & Swin-L & \multicolumn{1}{c|}{sup-21K} & 66.6 \\
%     \hline
%     \rowcolor{orange!50} \textbf{Plain detector} &  &  & \\
%     \multicolumn{1}{l|}{\ours} & ViT-B & \multicolumn{1}{c|}{MAE} & 66.6 \\
%     \multicolumn{1}{l|}{\ours} & ViT-L & \multicolumn{1}{c|}{MAE} & \textbf{67.2} \\
%     \end{tabular}
%     }
%     {
%         \caption{\textbf{More panoptic segmentation comparison on Cityscapes.} We compare between methods using feature pyramids (\emph{top} row) \vs single-scale (\emph{bottom} row) on Cityscapes~\val. \ours as the plain detector still shows competitive results.}\label{tab:cityscapes}
%     }%
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
% \boldparagraph{More panoptic segmentation comparison on Cityscapes.} We observe a similar trend in \cref{tab:cityscapes} that \ours shows good improvement when increasing the model size. \ours with ViT-L reaches the best performance of 67.2 PQ point, outperforming other multi-scale segmentation models.

==> sup/visualize.tex <==


\begin{figure}[h!]
    \footnotesize
    \centering
    
    % \begin{minipage}{0.45\textwidth}
    % \centering
    
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/success/val_111_det.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/success/val_111_pan.png}
    \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_358_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_358_pan.png}
    % \end{minipage}
    
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/success/val_159_det.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/success/val_159_pan.png}
    \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_63_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_63_pan.png}
    % \end{minipage}
    
    % \begin{minipage}[b]{.45\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_927_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.45\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_927_pan.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_896_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_896_pan.png}
    % \end{minipage}
    
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_486_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_486_pan.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_308_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_308_pan.png}
    % \end{minipage}
    
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/success/val_663_det.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/success/val_663_pan.png}
    \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_577_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_577_pan.png}
    % \end{minipage}
    
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/success/val_129_det.png}

    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/success/val_129_pan.png}

    \end{minipage}
    % \begin{minipage}[b]{.45\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_181_det.png}

    % {\footnotesize \text{\hspace{7em} Instance \par}}
    % \end{minipage}
    % \begin{minipage}[b]{.45\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_181_pan.png}

    % {\footnotesize \text{\hspace{7em} Panoptic \par}}
    % \end{minipage}
    
    % \end{minipage}
    
    \caption{\textbf{Qualitative results} generated by \ours using ViT-B as backbone on the COCO \val.}
    \label{fig:vis_sup}
\end{figure}


\begin{figure}[h!]
    \footnotesize
    \centering
    
    % \begin{minipage}{0.45\textwidth}
    % \centering
    
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_429.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_432.png}
    \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_358_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_358_pan.png}
    % \end{minipage}
    
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_474.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_480.png}
    \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_63_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_63_pan.png}
    % \end{minipage}
    
    % \begin{minipage}[b]{.45\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_927_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.45\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_927_pan.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_896_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_896_pan.png}
    % \end{minipage}
    
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_486_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_486_pan.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_308_det.png}
    % \end{minipage}
    % \begin{minipage}[b]{.245\linewidth}
    % \includegraphics[width=\linewidth]{vis/success/val_308_pan.png}
    % \end{minipage}
    
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_491.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_492.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_458.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_488.png}
    \end{minipage}
    
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_493.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_494.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_495.png}
    \end{minipage}
    \begin{minipage}[b]{.45\linewidth}
    \includegraphics[width=\linewidth]{vis/cs/val_498.png}
    \end{minipage}
    
    % \end{minipage}
    
    \caption{\textbf{Qualitative results} of panoptic segmentation generated by \ours on Cityscapes \val.}
    \label{fig:vis_sup_cs}
\end{figure}

\section{Qualitative results}

We provide qualitative results of the \ours prediction with ViT-B backbone on three tasks: COCO object detection, instance segmentation, and panoptic segmentation in \cref{fig:vis_sup}.

The visualization of panoptic segmentation on Cityscapes \val is also provised in \cref{fig:vis_sup_cs}.

% \section{Asset Licenses}

%##################################################################################################
\begin{center}
% \vspace{-.2em}
\tablestyle{4pt}{1.05}
%\scriptsize
\footnotesize
\begin{tabular}{l|l}
Dataset & License \\
\shline
ImageNet~\citep{deng2009imagenet}& \url{https://image-net.org/download.php} \\
COCO~\citep{lin2014mscoco}       & Creative Commons Attribution 4.0 License \\
Cityscapes~\citep{cordts2016cityscapes}       & \url{https://www.cityscapes-dataset.com/license} \\
\end{tabular}
% \vspace{-.2em}
% \vspace{-5pt}
\end{center}
%##################################################################################################

